Det6D: A Ground-Aware Full-Pose 3D Object Detector for Improving Terrain Robustness

Accurate 3D object detection with LiDAR is critical for autonomous driving. Existing research is all based on the flat-world assumption. However, the actual road can be complex with steep sections, which breaks the premise. Current methods suffer from performance degradation in this case due to difficulty correctly detecting objects on sloped terrain. In this work, we propose Det6D, the first full-degree-of-freedom 3D object detector without spatial and postural limitations, to improve terrain robustness. We choose the point-based framework by founding their capability of detecting objects in the entire spatial range. To predict full-degree poses, including pitch and roll, we design a ground-aware orientation branch that leverages the local ground constraints. Given the difficulty of long-tail non-flat scene data collection and 6D pose annotation, we present Slope-Aug, a data augmentation method for synthesizing non-flat terrain from existing datasets recorded in flat scenes. Experiments on various datasets demonstrate the effectiveness and robustness of our method in different terrains. We further conducted an extended experiment to explore how the network predicts the two extra poses. The proposed modules are plug-and-play for existing point-based frameworks. The code is available at https://github.com/HITSZ-NRSL/De6D.

==> _exp__fig_gazebo.tex <==
\begin{figure}
\centering
\subfigure[Scenes]{
    \begin{minipage}[b]{0.15\linewidth}
        \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/up_slope/up_slope_2.jpg}\vspace{2pt}
        \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/down_slope/down_slope_1.jpg}\vspace{2pt}
        \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/side_way/sideway_1.jpg}
    \end{minipage}
}\hspace{2pt}
\subfigure[PointPillars\cite{pointpillars}]{
    \begin{minipage}[b]{0.15\linewidth}
        \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/up_slope/pointpillars.png}\vspace{2pt}
        \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/down_slope/pointpillars.png}\vspace{2pt}
        \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/side_way/pointpillars.png}
    \end{minipage}
}\hspace{2pt}
\subfigure[Voxel R-CNN\cite{deng2020voxel}]{
    \begin{minipage}[b]{0.15\linewidth}
        \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/up_slope/voxel_rcnn.png}\vspace{2pt}
        \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/down_slope/voxel_rcnn.png}\vspace{2pt}
        \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/side_way/voxel_rcnn.png}
    \end{minipage}
}\hspace{2pt}
\subfigure[PointRCNN\cite{shi2019pointrcnn}]{
    \begin{minipage}[b]{0.15\linewidth}
        \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/up_slope/pointrcnn.png}\vspace{2pt}
        \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/down_slope/pointrcnn.png}\vspace{2pt}
        \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/side_way/pointrcnn.png}
    \end{minipage}
}\hspace{2pt}
\subfigure[Det6D(Ours)]{
    \begin{minipage}[b]{0.15\linewidth}
        \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/up_slope/det6d_sasa.png}\vspace{2pt}
        \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/down_slope/det6d_sasa.png}\vspace{2pt}
        \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/side_way/det6d_sasa.png}
    \end{minipage}
}
\caption{GAZEBO仿真中几个代表性场景的检测结果比较，自身车辆处于即将上坡(第一行)、在下坡中(第二行)、支路汇入中(第三行)。第一列为场景图(红圈为ego vehicle)，其余列为不同模型的检测可视化，绿框为检测结果。}
\label{fig:gazebo_viz}
\end{figure}


% \begin{figure}
% \centering
% \subfigure{
%     \begin{minipage}[b]{0.15\linewidth}
%         \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/up_slope/up_slope_2.jpg}\vspace{2pt}
%         \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/down_slope/down_slope_1.jpg}\vspace{2pt}
%         \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/side_way/sideway_1.jpg}
%     \end{minipage}
% }\hspace{2pt}
% \subfigure{
%     \begin{minipage}[b]{0.15\linewidth}
%         \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/up_slope/pointpillars.png}\vspace{2pt}
%         \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/down_slope/pointpillars.png}\vspace{2pt}
%         \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/side_way/pointpillars.png}
%     \end{minipage}
% }\hspace{2pt}
% \subfigure{
%     \begin{minipage}[b]{0.15\linewidth}
%         \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/up_slope/voxel_rcnn.png}\vspace{2pt}
%         \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/down_slope/voxel_rcnn.png}\vspace{2pt}
%         \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/side_way/voxel_rcnn.png}
%     \end{minipage}
% }\hspace{2pt}
% \subfigure{
%     \begin{minipage}[b]{0.15\linewidth}
%         \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/up_slope/pointrcnn.png}\vspace{2pt}
%         \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/down_slope/pointrcnn.png}\vspace{2pt}
%         \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/side_way/pointrcnn.png}
%     \end{minipage}
% }\hspace{2pt}
% \subfigure{
%     \begin{minipage}[b]{0.15\linewidth}
%         \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/up_slope/det6d_sasa.png}\vspace{2pt}
%         \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/down_slope/det6d_sasa.png}\vspace{2pt}
%         \includegraphics[width=1.0\linewidth]{img/gazebo_result/exp1/side_way/det6d_sasa.png}
%     \end{minipage}
% }
% \caption{GAZEBO仿真中几个代表性场景的检测结果比较，自身车辆处于即将上坡(第一行)、在下坡中(第二行)、支路汇入中(第三行)。第一列为场景图(红圈为ego vehicle)，剩的分别为PointPillars\cite{pointpillars}、Voxel R-CNN\cite{deng2020voxel}、PointRCNN\cite{shi2019pointrcnn}和Det6D(Ours)，绿框为检测结果。}
% \label{fig:gazebo_viz}
% \end{figure} 

==> _exp__fig_slopedkitti.tex <==
\begin{figure*}
\centering
\subfloat{%
    \setcounter{subfigure}{0}
    \begin{minipage}[]{0.002\linewidth}
        \rotatebox{90}{\tiny SlopedKITTI}
    \end{minipage}
}
\subfloat[CenterPoint\cite{yin2021center}\label{fig:slopekitti_viz:a}]{%
    \begin{minipage}[]{0.192\linewidth}
        \includegraphics[width=1\linewidth]{img/kitti_result/CenterPoint_2360_004721_0.png}\vspace{0.5pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/CenterPoint_2360_004721_1.png}\vspace{2pt}
        % \includegraphics[width=1\linewidth]{img/kitti_result/CenterPoint_26_000053_0.png}\vspace{0.5pt}
        % \includegraphics[width=1\linewidth]{img/kitti_result/CenterPoint_26_000053_1.png}\vspace{2pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/CenterPoint_3328_006664_0.png}\vspace{0.5pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/CenterPoint_3328_006664_1.png}\vspace{2pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/CenterPoint_67_000159_0.png}\vspace{0.5pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/CenterPoint_67_000159_1.png}\vspace{2pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/CenterPoint_96_000213_0.png}\vspace{0.5pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/CenterPoint_96_000213_1.png}
    \end{minipage}}
\hfill
\subfloat[PV-RCNN\cite{shi2020pv}\label{fig:slopekitti_viz:b}]{%
    \begin{minipage}[]{0.192\linewidth}
        \includegraphics[width=1\linewidth]{img/kitti_result/PVRCNN_2360_004721_0.png}\vspace{0.5pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/PVRCNN_2360_004721_1.png}\vspace{2pt}
        % \includegraphics[width=1\linewidth]{img/kitti_result/PVRCNN_26_000053_0.png}\vspace{0.5pt}
        % \includegraphics[width=1\linewidth]{img/kitti_result/PVRCNN_26_000053_1.png}\vspace{2pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/PVRCNN_3328_006664_0.png}\vspace{0.5pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/PVRCNN_3328_006664_1.png}\vspace{2pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/PVRCNN_67_000159_0.png}\vspace{0.5pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/PVRCNN_67_000159_1.png}\vspace{2pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/PVRCNN_96_000213_0.png}\vspace{0.5pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/PVRCNN_96_000213_1.png}
    \end{minipage}}
\hfill
\subfloat[Voxel R-CNN\cite{deng2020voxel}\label{fig:slopekitti_viz:c}]{%
    \begin{minipage}[]{0.192\linewidth}
        \includegraphics[width=1\linewidth]{img/kitti_result/VoxelRCNN_2360_004721_0.png}\vspace{0.5pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/VoxelRCNN_2360_004721_1.png}\vspace{2pt}
        % \includegraphics[width=1\linewidth]{img/kitti_result/VoxelRCNN_26_000053_0.png}\vspace{0.5pt}
        % \includegraphics[width=1\linewidth]{img/kitti_result/VoxelRCNN_26_000053_1.png}\vspace{2pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/VoxelRCNN_3328_006664_0.png}\vspace{0.5pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/VoxelRCNN_3328_006664_1.png}\vspace{2pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/VoxelRCNN_67_000159_0.png}\vspace{0.5pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/VoxelRCNN_67_000159_1.png}\vspace{2pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/VoxelRCNN_96_000213_0.png}\vspace{0.5pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/VoxelRCNN_96_000213_1.png}
    \end{minipage}}
\hfill
\subfloat[PointRCNN\cite{shi2019pointrcnn}\label{fig:slopekitti_viz:d}]{%
    \begin{minipage}[]{0.192\linewidth}
        \includegraphics[width=1\linewidth]{img/kitti_result/PointRCNN_2360_004721_0.png}\vspace{0.5pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/PointRCNN_2360_004721_1.png}\vspace{2pt}
        % \includegraphics[width=1\linewidth]{img/kitti_result/PointRCNN_26_000053_0.png}\vspace{0.5pt}
        % \includegraphics[width=1\linewidth]{img/kitti_result/PointRCNN_26_000053_1.png}\vspace{2pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/PointRCNN_3328_006664_0.png}\vspace{0.5pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/PointRCNN_3328_006664_1.png}\vspace{2pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/PointRCNN_67_000159_0.png}\vspace{0.5pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/PointRCNN_67_000159_1.png}\vspace{2pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/PointRCNN_96_000213_0.png}\vspace{0.5pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/PointRCNN_96_000213_1.png}
    \end{minipage}}
\hfill
\subfloat[Det6D(Ours)\label{fig:slopekitti_viz:e}]{%
    \begin{minipage}[]{0.192\linewidth}
        \includegraphics[width=1\linewidth]{img/kitti_result/Det6D_2360_004721_0.png}\vspace{0.5pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/Det6D_2360_004721_1.png}\vspace{2pt}
        % \includegraphics[width=1\linewidth]{img/kitti_result/Det6D_26_000053_0.png}\vspace{0.5pt}
        % \includegraphics[width=1\linewidth]{img/kitti_result/Det6D_26_000053_1.png}\vspace{2pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/Det6D_3328_006664_0.png}\vspace{0.5pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/Det6D_3328_006664_1.png}\vspace{2pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/Det6D_67_000159_0.png}\vspace{0.5pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/Det6D_67_000159_1.png}\vspace{2pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/Det6D_96_000213_0.png}\vspace{0.5pt}
        \includegraphics[width=1\linewidth]{img/kitti_result/Det6D_96_000213_1.png}
    \end{minipage}}
\hfill
\subfloat{%
    \begin{minipage}[]{0.002\linewidth}
        \rotatebox{90}{\tiny Scene 4 \hspace{30pt} Scene 3 \hspace{30pt} Scene 2 \hspace{30pt} Scene 1}
    \end{minipage}
}
\caption{
Visualization results on SlopedKITTI.
%Det6D和现存算法在SlopedKITTI数据集中非平面场景下的性能比较可视化。
Each row represents a different scene.
%不同行表示不同场景，不同列表示不同算法的结果。
In each result, the top image is the front view, and the bottom one is the side view showing the terrain.
%每个场景中上方的图片为前视图展示检测结果，下方为侧视图以展示地形。
The red box is the ground-truth, and the green box is the detection result.
%CenterPoint、PV-RCNN、Voxel R-CNN不能对斜坡上的车辆进行检测，而PointRCNN对斜坡上的物体无法正确估计位姿并且有大量的错误检测。可以注意到我们的方法还正确的检测到没标注的物体。
Please zoom in for details.}
\label{fig:slopekitti_viz}
\end{figure*} 


% \begin{figure*}
% \centering
% \subfigure{
% \begin{minipage}[b]{0.185\linewidth}
% \includegraphics[width=1\linewidth]{img/kitti_result/CenterPoint_2360_004721_0.png}
% \includegraphics[width=1\linewidth]{img/kitti_result/CenterPoint_2360_004721_1.png}\vspace{2pt}
% \includegraphics[width=1\linewidth]{img/kitti_result/CenterPoint_26_000053_0.png}
% \includegraphics[width=1\linewidth]{img/kitti_result/CenterPoint_26_000053_1.png}\vspace{2pt}
% \includegraphics[width=1\linewidth]{img/kitti_result/CenterPoint_3328_006664_0.png}
% \includegraphics[width=1\linewidth]{img/kitti_result/CenterPoint_3328_006664_1.png}\vspace{2pt}
% \includegraphics[width=1\linewidth]{img/kitti_result/CenterPoint_67_000159_0.png}
% \includegraphics[width=1\linewidth]{img/kitti_result/CenterPoint_67_000159_1.png}\vspace{2pt}
% \includegraphics[width=1\linewidth]{img/kitti_result/CenterPoint_96_000213_0.png}
% \includegraphics[width=1\linewidth]{img/kitti_result/CenterPoint_96_000213_1.png}
% \end{minipage}}
% \subfigure{
% \begin{minipage}[b]{0.185\linewidth}
% \includegraphics[width=1\linewidth]{img/kitti_result/PVRCNN_2360_004721_0.png}
% \includegraphics[width=1\linewidth]{img/kitti_result/PVRCNN_2360_004721_1.png}\vspace{2pt}
% \includegraphics[width=1\linewidth]{img/kitti_result/PVRCNN_26_000053_0.png}
% \includegraphics[width=1\linewidth]{img/kitti_result/PVRCNN_26_000053_1.png}\vspace{2pt}
% \includegraphics[width=1\linewidth]{img/kitti_result/PVRCNN_3328_006664_0.png}
% \includegraphics[width=1\linewidth]{img/kitti_result/PVRCNN_3328_006664_1.png}\vspace{2pt}
% \includegraphics[width=1\linewidth]{img/kitti_result/PVRCNN_67_000159_0.png}
% \includegraphics[width=1\linewidth]{img/kitti_result/PVRCNN_67_000159_1.png}\vspace{2pt}
% \includegraphics[width=1\linewidth]{img/kitti_result/PVRCNN_96_000213_0.png}
% \includegraphics[width=1\linewidth]{img/kitti_result/PVRCNN_96_000213_1.png}
% \end{minipage}}
% \subfigure{
% \begin{minipage}[b]{0.185\linewidth}
% \includegraphics[width=1\linewidth]{img/kitti_result/VoxelRCNN_2360_004721_0.png}
% \includegraphics[width=1\linewidth]{img/kitti_result/VoxelRCNN_2360_004721_1.png}\vspace{2pt}
% \includegraphics[width=1\linewidth]{img/kitti_result/VoxelRCNN_26_000053_0.png}
% \includegraphics[width=1\linewidth]{img/kitti_result/VoxelRCNN_26_000053_1.png}\vspace{2pt}
% \includegraphics[width=1\linewidth]{img/kitti_result/VoxelRCNN_3328_006664_0.png}
% \includegraphics[width=1\linewidth]{img/kitti_result/VoxelRCNN_3328_006664_1.png}\vspace{2pt}
% \includegraphics[width=1\linewidth]{img/kitti_result/VoxelRCNN_67_000159_0.png}
% \includegraphics[width=1\linewidth]{img/kitti_result/VoxelRCNN_67_000159_1.png}\vspace{2pt}
% \includegraphics[width=1\linewidth]{img/kitti_result/VoxelRCNN_96_000213_0.png}
% \includegraphics[width=1\linewidth]{img/kitti_result/VoxelRCNN_96_000213_1.png}
% \end{minipage}}
% \subfigure{
% \begin{minipage}[b]{0.185\linewidth}
% \includegraphics[width=1\linewidth]{img/kitti_result/PointRCNN_2360_004721_0.png}
% \includegraphics[width=1\linewidth]{img/kitti_result/PointRCNN_2360_004721_1.png}\vspace{2pt}
% \includegraphics[width=1\linewidth]{img/kitti_result/PointRCNN_26_000053_0.png}
% \includegraphics[width=1\linewidth]{img/kitti_result/PointRCNN_26_000053_1.png}\vspace{2pt}
% \includegraphics[width=1\linewidth]{img/kitti_result/PointRCNN_3328_006664_0.png}
% \includegraphics[width=1\linewidth]{img/kitti_result/PointRCNN_3328_006664_1.png}\vspace{2pt}
% \includegraphics[width=1\linewidth]{img/kitti_result/PointRCNN_67_000159_0.png}
% \includegraphics[width=1\linewidth]{img/kitti_result/PointRCNN_67_000159_1.png}\vspace{2pt}
% \includegraphics[width=1\linewidth]{img/kitti_result/PointRCNN_96_000213_0.png}
% \includegraphics[width=1\linewidth]{img/kitti_result/PointRCNN_96_000213_1.png}
% \end{minipage}}
% \subfigure{
% \begin{minipage}[b]{0.185\linewidth}
% \includegraphics[width=1\linewidth]{img/kitti_result/Det6D_2360_004721_0.png}
% \includegraphics[width=1\linewidth]{img/kitti_result/Det6D_2360_004721_1.png}\vspace{2pt}
% \includegraphics[width=1\linewidth]{img/kitti_result/Det6D_26_000053_0.png}
% \includegraphics[width=1\linewidth]{img/kitti_result/Det6D_26_000053_1.png}\vspace{2pt}
% \includegraphics[width=1\linewidth]{img/kitti_result/Det6D_3328_006664_0.png}
% \includegraphics[width=1\linewidth]{img/kitti_result/Det6D_3328_006664_1.png}\vspace{2pt}
% \includegraphics[width=1\linewidth]{img/kitti_result/Det6D_67_000159_0.png}
% \includegraphics[width=1\linewidth]{img/kitti_result/Det6D_67_000159_1.png}\vspace{2pt}
% \includegraphics[width=1\linewidth]{img/kitti_result/Det6D_96_000213_0.png}
% \includegraphics[width=1\linewidth]{img/kitti_result/Det6D_96_000213_1.png}
% \end{minipage}}
% \caption{Det6D和现存算法在非平面场景下的性能比较，从左到右分别是CenterPoint\cite{yin2021center}、PV-RCNN\cite{shi2020pv}、Voxel R-CNN\cite{deng2020voxel}、PointRCNN\cite{shi2019pointrcnn}和Det6D(ours)。每张图片的上方为前视图下的检测结果，下方为侧视图以显示地形。红色为真值框，绿色为检测结果。CenterPoint、PV-RCNN、Voxel R-CNN不能对斜坡上的车辆进行检测，而PointRCNN对斜坡上的物体无法正确估计位姿并且有大量的错误检测。可以注意到我们的方法还正确的检测到没标注的物体。Best view in color}
% \label{fig:slopekitti_viz}
% \end{figure*} 

